Transactional Panorama: A Conceptual Framework for User Perception in Analytical Visual Interfaces

Many tools empower analysts and data scientists to consume analysis results in a visual interface, such as a dashboard. When the underlying data changes, these results need to be updated, but this update can take a long time -- all while the user continues to explore the results. In this context, tools can either (i) hide away results that haven't been updated, hindering exploration; (ii) make the updated results immediately available to the user (on the same screen as old results), leading to confusion and incorrect insights; or (iii) present old -- and therefore stale -- results to the user during the update. To help users reason about these options and others, and make appropriate trade-offs, we introduce Transactional Panorama, a formal framework that adopts transactions to jointly model the system refreshing the analysis results and the user interacting with them. We introduce three key properties that are important for user perception in this context, visibility (allowing users to continuously explore results), consistency (ensuring that results resented are from the same version of the data), and monotonicity (making sure that results don't "go back in time"). Within transactional panorama, we characterize all of the feasible property combinations, design new mechanisms (that we call lenses) for presenting analysis results to the user while preserving a given property combination, formally prove their relative orderings for various performance criteria and discuss their use cases. We propose novel algorithms to preserve each property combination and efficiently present fresh analysis results. We implement our transactional panorama framework in a popular, open-source BI tool, illustrate the relative performance implications of different lenses, demonstrate the benefits of the novel lenses, and outline the performance improvement by our optimizations.

==> intro-bkp-July30.tex <==
\section{Introduction}
\label{sec:intro}

Many user-facing data analysis tools 
empower users to visually organize, present, and consume the 
results of multiple types of analysis in a single interface, 
such as a dashboard. 
Each analysis result is computed from the source data 
or other analysis results using relational operators, 
pandas dataframe expressions, spreadsheet formulae, 
and UDFs, akin to a database view. 
For example, in a business intelligence (BI) tool 
(e.g., Tableau~\cite{tableau}), 
users define the views from database tables using SQL statements
and visualize the views in a dashboard. 
Similarly, a workflow orchestration tool 
(e.g., Airflow~\cite{airflow} or Dagster~\cite{dagster}) 
allows users to build a data pipeline 
and visualize the results 
using a dashboarding tool (e.g., Streamlit~\cite{streamlit}). 
In a spreadsheet system, users define their computations 
via formulae and visualize the results in a tabular interface. 

In many scenarios, the views and the 
corresponding visualizations need to be refreshed 
when the source data is modified. 
For example, a dashboard in a BI tool 
will be refreshed 
with respect to the regular changes to base tables in the database 
(e.g., incorporating batches of new data). 
%When a user explores a dataset in  a BI tool, 
%they may also apply filters on the base tables 
%to refresh the visualizations and interactively investigate 
%the results for different subsets of the data. 
Similarly, in a spreadsheet system, a user often modifies the 
contents of individual cells to refresh the results of 
other downstream formulae that depend on the modification. 

%in a computational notebook, users will 
%also modify the contents of cells to refresh the results 
%of other cells that depend on the modification. 

%Unfortunately, when processing the updates on a \viewG and 
%refreshing the views, 
%many existing systems do not allow users to interact 
%with the system, leading to long response time 
%and significantly diminished interactivity. 
%For example, the BI tools Superset and Tableau 
%do not allow users to interact with a visualization and modify 
%the filters while they are refreshing the visualizations. 
% In addition, 
% Excel is frozen when it is recalculating the formulae~\cite{}. 

%\igc{The writing is really good in quality! The one comment I have at this point in the intro is that the next para is introducing the problem without having talked about: a) aspects of scale (of the dataset/spreadsheet/view graph), and b) the intensity of the computations that mean that the "spreading" of teh computation across the sheet is not instantaneous, and c) the user-facing impact of this slowness.}
%to express their 
%computations using a \df model~\cite{}, 
%where each computation, akin to a database view, 
%is defined on the source data or 
%the results of other computations using relational operators, 
%pandas dataframe, and UDFs, 
%creating a directed acyclic graph. 
%Each computation in this graph can be generally regarded as a view 
%and the graph is called a \textit{\viewG}. 

\begin{table}[t]
\fontsize{6.5}{8}\selectfont
\begin{tabular}{llccc}
\RealApproach                                                                   & Example Tools                                                            & \multicolumn{1}{l}{Monotonicity} & \multicolumn{1}{l}{Visibility} & \multicolumn{1}{l}{Consistency} \\ \hline
\begin{tabular}[c]{@{}l@{}}Globally-Consistent\\ Fully-Blocking (\pGCFB)\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}MS Excel~\cite{msexcel}\\ Libre Calc~\cite{libreCalc}\\ Tableau~\cite{tableau}\end{tabular}  & Yes                              & No                             & Yes                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Globally-Consistent\\ Partially-Blocking (\pGCPB)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Power BI~\cite{powerBI}\\ Superset~\cite{superset}\\ Dataspread~\cite{Antifreeze}\end{tabular} & Yes                              & No                             & Yes                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Inconsistently\\ Non-Blocking (\pICNB)\end{tabular}       & Google Sheets~\cite{sheets}                                                            & Yes                              & Yes                            & No                              \\ \hline
%\begin{tabular}[c]{@{}l@{}}Locally-consistent\\ Non-blocking (\pLCNB) {[}{]}\end{tabular} & None                                                                     & No                               & Yes                            & Yes                             \\ \hline
%\begin{tabular}[c]{@{}l@{}}Globally-consistent\\ Non-blocking (\pGCNB) {[}{]}\end{tabular} & None                                                                     & Yes                               & Yes                            & Yes                             \\ \hline
\end{tabular}
\caption{\small Properties maintained and sacrificed by existing tools}
\label{tbl:existing_work}
\vspace{-7mm}
\end{table}

\begin{figure}[!t]
    \centering
    \includegraphics[width=85mm]{figures/visual_examples_new.pdf}
    \vspace{-3mm}
    \caption{Visual examples of different \approaches of refreshing views in a dashboard}
    \label{fig:existing_tools}
    \vspace{-7mm}
\end{figure}

With the underlying dataset becoming larger 
and the analysis being more complex, 
it is time-consuming to refresh all of the views on one screen. 
Therefore, the concurrency between the system refreshing the 
views and the user exploring the results for different visualizations 
creates a key research question: 
\emph{how to present fresh and coherent results to a user 
without blocking the user from inspecting different visualizations}.
%\igc{alternate: \emph{how to present fresh and consistent results to a user without blocking the user from inspecting  any part of the visualization}. Recommend avoiding negative terms like non-confusing in a definition.}
%\igc{I'd recommend using ``user'' (singular) rather than users (plural) throughout the paper. Otherwise reviewers might ask about multiple users simultaneously interacting with the viz, which is not our target at all.}

Unfortunately, existing tools commonly make fixed and 
somehow arbitrary choices on optimizing some aspects 
of this research question 
and sacrificing others that could have been desired by a user, 
and the user does not have the freedom to make appropriate trade-offs. 
For example, existing tools~\cite{msexcel, libreCalc, tableau, powerBI, superset} present coherent results across space and time dimensions 
by maintaining two properties: \emph{\con} and \emph{\mon}. 
\Con guarantees the analysis results 
displayed on the screen should be consistent 
with the same snapshot of source data~\cite{GolabJ11Consistency, ZhugeGW97Multiview}. 
\Mon guarantees if a user reads the result 
for a view, any successive read on this view will always 
return the same or more recent result (i.e., monotonic read~\cite{DSBook}). 
To maintain the two properties, one \realApproach 
blocks the user from interacting with the system 
until the system has finished updating all of the views related 
to the source data modification, as shown by the first visual example 
in Figure~\ref{fig:existing_tools}. 
This \realApproach is adopted by Excel~\cite{msexcel}, Libre Calc~\cite{libreCalc}, and Tableau~\cite{tableau} and is referred to 
as \emph{\GCFB} (\emph{\pGCFB} for short). 
However, the problem of \pGCFB is that the user cannot 
interact with the visualizations for significant periods of time. 
To mitigate this problem, another \realApproach 
proposes initially marking the views  
that depend on the update \unavailable 
and making each view \available only 
when the system has computed its new result~\cite{Antifreeze}. 
We denote this \realApproach as \textit{\GCPB} (\emph{\pGCPB} for short) 
and a visual example is shown in Figure~\ref{fig:existing_tools}. 
This \realApproach is adopted in BI tools, 
such as PowerBI~\cite{powerBI} and Superset~\cite{superset}, 
and a spreadsheet tool, Dataspread~\cite{Antifreeze}. 
However, both \pGCFB and \pGCPB maintain \con and \mon 
by sacrificing \textit{\ava}, 
a property that ensures interactivity 
by guaranteeing a user always sees 
and interacts with the result of any visualization. 

On the other end of the spectrum is an \realApproach 
that maintains \ava by sacrificing \con. 
We denote this \realApproach as \emph{\ICNB} or \emph{\pICNB} for short. 
Specifically, \pICNB always allows a user to 
inspect the result of any visualization, no matter its freshness,  
and makes the new result \available to the user 
immediately after the system has computed it, 
sacrificing \con. 
For example, if we refresh visualizations on the screen 
with respect to the modification to one base table, 
some visualizations will be up-to-date with the new base table 
while others will be consistent with the old one, 
rendering inconsistent results, 
as shown in Figure~\ref{fig:existing_tools}. 
\pICNB is adopted by Google Sheets~\cite{sheets}.
Finally, as we show in this paper, it is possible 
to achieve both \con and \ava simultaneously 
only by either sacrificing \mon or suffering from 
high \snMetric, which means there will 
be a long time when the analysis results a user sees 
are not consistent with the new source data 
(i.e., stale results).

%\igc{I love Fig \ref{fig:trade-off_full}. We should be referring it at more points in the text of this section (especially at points we introduce GF, GP, IN,... and also justify why they sit there. This justification is there right now for some of these in the text, but not consistently or clearly so.}

%\igc{Might help to have a table summarizing the definitions of GF, GP, IN,... For readers to quickly reference as they read the rest of the paper.}

\begin{figure}[!t]
    \centering
    \includegraphics[height=35mm]{figures/trade-off-full.pdf}
    \vspace{-3mm}
    \caption{Trade-off between \uaMetric and \snMetric across different property combinations}
    \label{fig:trade-off_full}
    \vspace{-5mm}
\end{figure}

In addition, the aforementioned \realApproach{es}
have different performance implications and 
a user should have the freedom to make the performance trade-offs, 
which is shown in Figure~\ref{fig:trade-off_full}. 
Specifically, \pGCFB blocks a user from interacting 
with the views until all of the new \res{s} are computed, 
so it has high \textit{\uaMetric}: a long time when 
the user cannot see and interact with the visualizations. 
But \pGCFB has zero \snMetric since 
it does not present stale results to the user. 
\pGCPB reduces \pGCFB's \uaMetric by presenting the newly computed 
\res{s} to the user whenever they are computed 
and also does not have stale results. 
\pICNB, the \realApproach that sacrifices \con, 
has higher \snMetric because the user can read stale results, 
but it does not include \unavailable views (i.e., zero \uaMetric).

%\igc{One thing that may not be clear to the reader is what a transaction looks like. Or whether transactions are the common ways the user in fact interacts with such a system. If it is common, we should say so and give an example. If it is sth new we are proposing (for viz systems), we need to motivate it. In either case, right now, the introduction of transactions kinda comes out of nowhere.}

To systematically reason about the property space 
and the related performance, 
we introduce a new \model, \emph{\tdb}.
It adopts \txn{s} to jointly model the system 
updating the visualizations 
and the user exploring the results for different visualizations, 
formally defines the properties \mon, \ava, and \con (or \macPro), 
studies the feasibility of different property combinations, 
and unveils their performance trade-offs. 
In \tdb, we name an \realApproach that adopts one property combination
a \emph{\approach}, which represents the way we present results 
to the user in a dashboard. 
We highlight \emph{\tdb is the first model that leverages 
\txn{s} to model a user's behaviors in visual interfaces}. 

%\igc{Is this too much detail for the Introduction? This paragraph was hard to read, as it introduces a lot of ideas without presenting any details. Not sure if moving this to a new Section 2 called Summary of TraVis, or sth similar, might address this.}
With \tdb, we can \emph{discover new property combinations} 
that have not yet been considered in existing tools. 
We then build a system that \emph{allows a user to 
choose different properties and 
make different performance trade-offs they desire}. 
Specifically, \tdb introduces three new \approaches: 
\GCNB (\pGCNB), \LCNB (\pLCNB), and \LCMB (\pLCMB), 
which adopt different newly discovered property combinations 
and have different performance implications. 
For example, \pLCNB always allows the user to inspect the results 
of any visualizations (i.e., preserving \ava), 
and refreshes the visualizations on the screen 
when all of their new results are computed (i.e., preserving \con). 
Figure~\ref{fig:existing_tools} shows an example of \pLCNB, 
where the user can quickly read the new results 
on the screen (i.e., $View_{1-4}$) without waiting 
for computing the new results that 
are not on the current screen (i.e., $View_{5-6}$). 
\pLCNB is used when a user wants to always see 
and interact with consistent results on the screen. 
However, as we prove later, \pLCNB needs to sacrifice \mon 
when the user explores different visualizations 
(e.g., scrolling the mouse). 
For the aforementioned new \approaches, 
we further introduce the $k$-\relaxed variants
(i.e., \kGCNB, \kLCNB, and \kLCMB), where 
$k$ represents the number of additional \unavailable views 
allowed for respective \approaches. 
These \approaches allow a user to gracefully 
explore the trade-off between \snMetric and \uaMetric. 
We summarize the new \approaches and their performance trade-offs 
in Figure~\ref{fig:trade-off_full} and will discuss them in detail 
later. To realize \tdb, we need to address the following challenges. 
%For example, one \approach of maintaining all of \macPro 
%is allowing the user to explore the old results 
%and refreshing the dashboard when all of the new results 
%are computed, as the example in Figure~\ref{fig:existing_tools} shows. 
%This \approach is referred to as \emph{\GCNB} or \emph{\pGCNB}. 
%As Figure~\ref{fig:trade-off_full} shows, 
%it has high \snMetric because the user reads stale results 
%until all of the new results are computed. 
%Another \approach that reduces \snMetric is to 
%allow the user to explore the old results 
%and refresh the results on the screen 
%when they are computed 
%without waiting for other results being up-to-date 
%(denoted \emph{\LCNB} or \emph{\pLCNB}). 
%One example of \pLCNB is shown in Figure~\ref{fig:existing_tools}, 
%where we refresh the results for \code{View~{1-4}} on the screen 
%when their new results are computed, 
%but do not have to wait for the new results for \code{View~{5-6}}. 
%As we prove later, when a user explores other views 
%that are not originally on the current screen, 
%\pLCNB needs to sacrifice \mon. 
%To maintain \mon, and achieve low \snMetric 
%and \uaMetric simultaneously, 
%we propose a \pLCNB variant: \emph{\LCMB} or \emph{\pLCMB} for short. 
%\pLCMB allows the \emph{minimum}
%number of \unavailable views on the screen to preserve \mon. 
%The trade-offs made by \pLCNB and \pLCMB are shown 
%in Figure~\ref{fig:trade-off_full}. 
%In addition to the three new \approaches \pGCNB, \pLCNB, 
%and \pLCMB, we introduce their $k$-\relaxed versions: 
%allowing $k$ more \unavailable views for each \approach 
%to refresh the results 
%(i.e., \kGCNB, \kLCNB, and \kLCMB 
%in Figure~\ref{fig:trade-off_full}). 
%The $k$-\relaxed versions enable users to further explore 
%the trade-off between \uaMetric and \snMetric. 

First, in a visual interface the user does not explicitly submits 
\txn{s} as in traditional databases, 
but reads the views by looking at the screen. 
In addition, the user can read different subsets of views 
by changing the views on the screen. 
Therefore, the challenge here is to adapt \txn{s} to 
model the user's behaviors, an aspect not considered in existing works. 

The second challenge lies in defining \macPro. 
One unique requirement in visual interfaces 
is that a user wants to quickly read the new results for some views 
before the system computes all of the new results. 
If we model an update along with refreshing the related views 
as a \txn (to preserve \con), 
the user essentially wants to read the 
results of an \emph{uncommitted \txn}. 
How to define \mon, \ava, and \con for reading uncommitted results 
is not considered by traditional databases and 
needs to be addressed in our model. 
%Given \macPro defined, one additional challenge is to 
%evaluate the feasibility of preserving different property combinations 
%and discover new property combinations. 

Finally, \tdb requires defining new performance metrics 
that consider the unique semantics of visual interfaces, 
including the time of a view being \unavailable 
or a \available view being stale when it is read by a user. 
With the new performance metrics defined, 
we also need to theoretically understand the relative performance 
across different property combinations 
and design new algorithms to optimize the performance. 

%will be visible to users, which is different from many databases 
%where only committed data can be read 
%(i.e., read committed isolation level~\cite{}). 
%This \chara raises the challenge of avoiding transaction abortion 
%since their intermediate results are already seen by users. 
%In addition, defining \con over uncommitted data is also 
%not considered in existing research and should be addressed in our model. 

We address these challenges in \tdb. 
%and build \ace, 
%a system that adopts the \tdb model for a BI tool. 
It models reads and writes on the views as \txn{s}.  
Specifically, it introduces a special read-only \txn 
to model a user reading the views on the screen. 
This \txn does not block waiting for the new result of a view 
if the new result is not computed, 
but immediately returns an \unavailable state, 
indicating the result is under computation. 
To model the fact that the user keeps ``reading'' the views, 
the \readTxn is periodically issued to pull fresh results. 
On the other hand, a write on the source data along with 
refreshing the related views is modeled as a \writeTxn. 
Based on this abstraction, we define \macPro for \readTxn{s}, 
and include a series of theorems, called \textit{\macThe}, 
to find the possible property combinations, 
some of which are newly discovered combinations. 
We further define two performance metrics, \emph{\uaMetric 
and \snMetric}, and demonstrate 
the performance trade-offs across different property combinations. 
\UaMetric represents the total time of the views read by users 
being \unavailable and \snMetric represents 
the total time of the views read by users being stale. 
We present the \tdb model in Section~\ref{sec:model}. 

Based on \tdb, we build a system, \ace, intended for use with a BI tool. 
\ace allows a user to choose different \approaches 
that maintain different properties with different performance. 
In \ace, we design efficient algorithms for processing \readTxn{s} 
and maintaining the properties selected by users, 
and propose optimizations to reduce \uaMetric and \snMetric 
for processing \writeTxn{s}. 
The system design of \ace is presented in Section~\ref{sec:system}. 
We implement \ace in Superset, 
a popular open-source BI tool~\cite{superset}. 
Our experimental results in Section~\ref{sec:experiment} 
reveal the significant performance difference  
across different \approaches, 
and demonstrate the values of the new \approaches  
and the model that enables these options. 
In addition, the experiments show our optimizations can 
significantly reduce \uaMetric and \snMetric 
compared to the baseline (by up to 70\% and 75\%, respectively).  
Finally, we discuss the related work in Section~\ref{sec:related} 
and conclude the paper in Section~\ref{sec:conclusion}. 


==> revision.tex <==
%!TEX root = main.tex

\noindent {\huge \bf Summary for Revised Paper \#433 ``\fullTdb: A Conceptual Framework for User Perception in Analytical Visual Interfaces''}

We thank the reviewers and meta-reviewer for their 
careful review of our paper and their helpful comments. 
We have thoroughly revised the paper based on their suggestions. 
We first summarize the major changes 
and then discuss the detailed changes for each review one by one. 
To aid the review of our changed text in the main paper, 
we have highlighted major text revisions using a \rtwo{blue font}, 
added line numbers, and use \fpointer{x}{y}{z} to refer to 
a given line in the revised paper.

We have made the following major changes:
\begin{itemize}
    \item {[Terminology and Notation]}
    We refactored or more clearly 
    defined terminology used in the paper, 
    and added a table (Table~\ref{tbl:notation}) 
    for summarizing frequently used 
    notation in Section~\ref{sec:bg}-\ref{sec:formalize}.
    
    \item {[Properties and \Approach{es}]}
    We added a discussion for how \macPro are related 
    to correctness and performance in Section~\ref{sec:macPro}. 
    To explain different \approach{es} better, 
    we heavily refactored Section~\ref{sec:new_property} 
    and added a new figure and an associated example  (Figure~\ref{fig:timeline}) to illustrate 
    the differences.
    
    \item {[User Actions]} We added a new subsection (i.e., Section~\ref{sec:extension}) to discuss how \tdb can support 
    multiple user-driven actions beyond modifying the viewport.
    
    \item {[Scheduling Metric]} 
    We heavily revised Section~\ref{sec:scheduler} 
    to explain why the scheduling heuristic metric $\Metric_{k}^{t_i}$ 
    is effective in reducing \uaMetric and \snMetric 
    for all \approach{es} except \pGCNB 
    and added a formal definition for $\RTime_{k}^{t_i}$, 
    the total time during which a view $\vt_k$ has been read 
    in the viewport since the \writeTxn $\txw^{t_i}$ started, 
    a discussion on how to estimate $\RTime_{k}^{t_i}$,  
    and an intuitive explanation for 
    when and why $\RTime_{k}^{t_i}$ is a good heuristic metric 
    for reducing \uaMetric and \snMetric in Section~\ref{sec:scheduler}.
    
    \item {[Triggering Refreshes]} We added a discussion 
    for how to trigger a refresh in Section~\ref{sec:system} and Section~\ref{sec:prototype}. 
    
    \item {[Experimental Setup and Multiple New Experiments]} 
    We clarified the reason for why our focus is on 
    testing one refresh  
    and added an experiment (Figure~\ref{fig:exp_refresh_interval}) for testing multiple refreshes. 
    We added a discussion on how to estimate \snMetric and \uaMetric. 
    We also added experiments to compare our scheduling algorithm with one 
    scheduling algorithm based on performance metrics (Figures~\ref{fig:exp_opt_sl}-\ref{fig:exp_opt_iv}).
    All these changes are in Section~\ref{sec:experiment}. 
    
    \item {[Colors]} 
    We have changed the red and green colors to gold and blue, respectively.
    
\end{itemize}

\subsection*{Meta-review}
\Rev{M1, M2}{Address reviewer 1's questions / concerns about the treatment of dimensions; consider adding additional justification for the choice of scheduling heuristic}

\Ans{We now present the multiple dimensions of the \tdb model better, including adding a discussion for how the \macPro are related to correctness and performance. 
We also refactored Section~\ref{sec:new_property} to separately discuss GC-related \approach{es} and IC/LC-related \approach{es} (\textbf{R1.\{W1, D1, D4\}}). In addition, 
we have clarified the scheduling metric and 
added experiments (Figures~\ref{fig:exp_opt_sl}-\ref{fig:exp_opt_iv}) to compare our metric with an additional metric 
suggested by Reviewer \#1 (\textbf{R1.\{W2, D5\}}).}

\Rev{M3}{address reviewer 2's questions /concerns 
from the detailed comments section}

\Ans{In response to these concerns, 
we have now addressed the color issue, added a discussion 
     for how our system triggers refreshing the dashboard, 
     explained the reason for testing one refresh, 
     added an experiment to test multiple refreshes (Figure~\ref{fig:exp_refresh_interval}), 
     and refactored or more clearly defined the terminology
     we use in the paper (\textbf{R2}).}
     
\Rev{M4, M5}{answer reviewer 3's questions posed in W1 and W2, 
improve the writing in terms of clarity (e.g., reviewer 3 D2)}

\Ans{We have now clarified that the difference on 
    \uaMetric and \snMetric will be more significant when the user explores more visualizations (\textbf{R3.W1}), explained the method for measuring \snMetric and \uaMetric (\textbf{R3.\{W2, D1\}}), and added a table to summarize the frequently used notation in the paper (\textbf{R3.\{W3, D2\}}).}

%related to 
%reviewer~1 using an \rone{orange font}, 
%reviewer~2 using a \rtwo{blue font}, 
%and reviewer~3 using a \rthree{green font}. 
%In addition, we have highlighted revisions 
%for multiple reviewers with a \rmulti{purple font}.

\subsection*{Reviewer \#1}
\Rev{R1.W1}{Presentation and treatment of dimensions in the spectrum could be simplified. (D1, D4)}

\Ans{Please see the responses to \textbf{R1.D1} and \textbf{R1.D4}.}

\Rev{R1.W2}{More justification, analysis for the scheduling heuristic (D5)}

\Ans{Please see the response to \textbf{R1.D5}.}

\Rev{R1.D1}{The paper discusses a couple of interesting properties of interest: monotonicity, visibility, consistency, staleness, scope (global vs. local). I don't see a clear distinction between correctness vs. performance properties and it would be good to add that for clarity. E.g. monotonicity is a correctness property (ie. a lens that is not monotonic is not useful) whereas consistency, staleness and visibility are part of the design trade-offs.}

\Ans{We now discuss how \macPro are related 
to correctness and performance at the end of 
revised Section~\ref{sec:macPro} (\fpointer{5}{2}{438}). 
Specifically, both \mon and \con impact correctness, 
i.e., maintaining one or both of these properties 
may be essential to guaranteeing correct insights 
from the visual interface, depending on the application. 
The former ensures that users are not deceived by updates 
that get ``undone'', while the latter ensures that users 
viewing multiple visualizations on a screen can draw correct 
joint inferences based on the same snapshot of the source data. 
On the other hand, all of the \macPro impact performance 
since maintaining these properties will increase 
\snMetric and/or \uaMetric as we show in Section~\ref{sec:order}. 
Users can further make 
performance trade-offs between \uaMetric and \snMetric 
by choosing which \version of the \viewG to read 
(i.e., \newG, \oldG, or the one with the minimal number of 
\ua{s} for the viewport).
%\Ava, on the other hand, is only related to performance. 
%Maintaining \ava will however have high \snMetric. 
%Users can choose to sacrifice \ava or maintain a 
%constrained level of \uaMetric 
%(i.e. a controlled number of \ua{s}) to reduce \snMetric.}

We do not view scope as a property that is varied 
since all three types of consistencies 
(i.e., \cf, \cc, and \cm) are defined on the local scope. 
That is, the \con property is defined for \readTxn{s}, 
which are modeled as reading the views in the viewport 
(i.e., the local scope).
We include ``Globally Consistent (GC)'' 
in the names of the \approach{es} \pGCNB and \pGCPB 
only because \pGCNB and \pGCPB always 
read the \oldAndNew \viewG, respectively, 
and the resulting effect is that all of the \res{s} 
(in the viewport or otherwise) 
are consistent with a single \version of the \viewG. 
We have now clarified this point when we 
define \pGCPB and \pGCNB in Section~\ref{sec:new_property} 
(\fpointer{6}{1}{502}).}
%In addition, 
%\tdb only considers the local scope 
%because all of the three types of consistencies 
%(i.e., \cf, \cc, and \cm) are defined for \readTxn{s}, 
%which are modeled as reading the views in the viewport. 
%The \approach{es} \pGCPB and \pGCNB include ``GC'' in their 
%names because the two \approach{es} always present 
%the \qres{s} for \oldAndNew \pG, respectively, across 
%the visual interface. We have now clarified the reasons 
%for including ``GC'' in names of \pGCPB and \pGCNB 
%in Section~\ref{sec:new_property} (\fpointer{1}{2}{3}).}

\Rev{R1.D2}{Can you elaborate more on the user-perceived difference between Globally consistent vs. locally consistent lenses? Is there a trade-off between the two or is LC lens always better it always has either lower staleness or higher visibility compared to GC?}

\Ans{As mentioned in the response to \textbf{R1.D1}, 
the differences between the three types of consistencies 
(i.e., \cf, \cc, and \cm) stem 
from different choices in which \version of the \viewG 
is read. So, for different \approach{es} that preserves \con, 
the \res{s} in the viewport are by definition consistent 
and there is no perceived difference in terms of \con. 
However, the user will perceive different levels of \uaMetric 
and \snMetric for different \approach{es}. 
In the revised paper, we have clarified the user-perceived 
differences after we have defined 
each \approach in Section~\ref{sec:new_property} (\fpointer{6}{2}{527}).}

\Ans{In terms of the trade-offs between globally and 
locally consistent \approach{es}, we have formalized 
the performance trade-offs across all \approach{es}, 
as summarized in Figure~\ref{fig:order}. 
Specifically, for \snMetric, we have 
$S(\pGCPB) \leq S(\pLCMB) \leq S(\pLCNB) \leq S(\pGCNB)$, 
where $S(A)$ represents the \snMetric for a \approach $A$. 
For \uaMetric, we have $I(\pGCPB) \geq I(\pLCMB) 
\geq I(\pLCNB) = I(\pGCNB)$, where $I(A)$ represents 
the \uaMetric for a \approach $A$. 
So the LC \approach{es} are in fact ``sandwiched'' 
between the GC \approach{es} 
and do not dominate them. 
We have now added text for connecting 
the definitions of different \approach{es} to 
their relative performance trade-offs 
after we have defined 
each \approach in Section~\ref{sec:new_property} (\fpointer{6}{2}{531}).}

\Rev{R1.D3}{Is it true that $C_m$ = $C_c$ for the case when viewport does not change?}

\Ans{Even when the viewport does not change, \cm is not equivalent to 
\cc. Consider the example in Figure~\ref{fig:multiversion}, 
where $\vt_1$ is modified, triggering updates to $\vt_{3-6}$. 
Say the viewport includes $\vt_{3-5}$ and does not change. 
If \cc is adopted, we will read the new \res{s} for 
$\vt_{3-5}$ after the new \res{s} for $\vt_{3-6}$ are computed. 
However, for \cm, we will read the new \res{s} 
for $\vt_{3-5}$ after the new \res{s} for $\vt_{3-5}$ are computed, 
without having to wait for $\vt_{6}$ being computed. 
This is because reading the new \res{s} for $\vt_{3-5}$ 
does not return $\ua{s}$. 
In our revised paper, we have refactored our example 
to explain $\cm$ better and clarify this point (\fpointer{5}{2}{429}).}

\Rev{R1.D4}{One difficulty with the presentation is in the treatment of viewport in the formal analysis. If the viewport does not change, we have a much simpler spectrum (e.g GC = LC, $C_c$ = $C_m$) and would have simplified the analysis to begin with. Then extending that model to when the viewport could change may have aided comprehension. Sec 2.6 essentially depicts a spectrum with so many variables (consistency, scope, visibility, relaxation) making it harder to analyze.}

\Ans{As mentioned in the response to \textbf{R1.D3}, when the 
viewport does not change, \cc is not equivalent to \cm. 
In addition, the \approach{es} that adopt \cc and \cm
(e.g., \pGCNB and \pLCNB) will have different behavior 
even if the viewport does not change. 
We have added a new figure, Figure~\ref{fig:timeline}, 
which shows how different \approaches present different \res{s} 
over the time. 
We see that even when the viewport does not change (for the 
first 4 actions), \pGCNB and \pLCNB present different \res{s} 
to the user. So dividing it up based on the viewport dimension 
does not amount 
to a simplification of the analysis. However, the reviewer's point 
around improving comprehension still stands. 
Instead of dividing the discussion into cases 
based on whether the viewport changes, we have now refactored Section~\ref{sec:new_property} 
in the following ways: 1) we discuss the definitions of 
GC-related \approach{es} and IC/LC-related \approach{es} separately; 
2) after we have defined each \approach, we discuss 
the \approach{es} that are covered in existing tools 
and those that are newly discovered; 
3) finally, we discuss the variants for the new \approach{es}.}

\Rev{R1.D5}{There is not much information on how/why the scheduling algorithm is a good heuristic. How is the likelihood ie. $D^{t_i}_k$ estimated? Why is this a good heuristic? Is this a good heuristic for all lenses in the spectrum and is there an intuitive reasoning for that? Does using the performance metrics directly in the scheduling heuristic yield better results? Why are NoOpt and AntiFreeze good baselines for comparison?}

\Ans{We have now revised Section~\ref{sec:scheduler} 
to explain why the scheduling heuristic metric 
$\Metric_{k}^{t_i}$ is effective in reducing \uaMetric and \snMetric 
for all \approach{es} except \pGCNB. 
The \uaMetric and \snMetric of \pGCNB is 
independent of the scheduling order 
since \pGCNB will only read the \newG after all of the views are updated. 

We have added a formal definition for 
$\RTime_{k}^{t_i}$, which represents 
the total time during which a view $\vt_k$ has been 
read in the viewport since the \writeTxn $\txw^{t_i}$ started. 
We also added a discussion for how to estimate $\RTime_{k}^{t_i}$  
and an intuitive explanation for 
when and why $\RTime_{k}^{t_i}$ is a good 
at reducing \uaMetric and \snMetric for 
all \approach{es} except \pGCNB in Section~\ref{sec:scheduler}. 
Specifically, based on the definitions of the metrics, 
prioritizing computing the new \res{s} 
for the views that a user will spend more time on reading 
will best reduce \snMetric and \uaMetric. 
We use $\RTime_{k}^{t_i}$ as a proxy to predict the 
amount of time the user will spend on reading a view in the future 
based on the assumption that the user 
has {\em temporal locality} for reading view{s}.
The temporal locality assumption states that 
the user will spend more time on a view 
in the future if they spent more time on this view in the past. 
As this temporal locality assumption weakens, $\RTime_{k}^{t_i}$ 
will be less effective in reducing \uaMetric and \snMetric, 
as is verified by our 
experiments in Section~\ref{sec:exp_optimizations}. 

Finally, we have now added an experiment that uses the performance 
metrics as the scheduling metric in Section~\ref{sec:exp_optimizations} 
and explained the 
reasons for why we use \noOpt and \execOpt as the baselines.
Specifically, the new baseline (denoted as \metricOpt) 
prioritizes computing the view that introduces the 
most \uaMetric plus \snMetric. 
Since the \uaMetric and \snMetric are increased 
only when a view is read, \metricOpt effectively prioritizes computing 
the view that the user spent the most time reading, 
which corresponds to $\RTime_{k}^{t_i}$ in our scheduling metric. 
Therefore, \metricOpt also takes advantage of 
the temporal locality of the workload. 
Our experiments in Figure~\ref{fig:exp_opt_sl}-\ref{fig:exp_opt_iv} 
show that when there is strong temporal locality, 
\metricOpt and our metric have similar performance. 
But when the temporal locality weakens, our metric 
yields lower \snMetric and \uaMetric compared to \metricOpt 
since it additionally considers the 
different execution times for refreshing different views. 
We choose \noOpt and \execOpt as baselines because \noOpt 
represents the behavior from Superset while 
\execOpt is drawn from existing work that 
schedules refreshing views in a \viewG. }

\Rev{R1.D6}{P5, C1, L1-3: the text here is confusing. What does "preserving visibility requirement being stringent" mean?
P5. If space allows, it maybe useful to explain the different consistencies using a timeline with what happens when each additional view is computed}

\Ans{For the text in the original P5, C1, L1-3, we wanted to highlight 
that a user can sacrifice \ava and opt for partial \ava, where they 
accept a controlled number of \ua{s} 
as a trade-off for reading fresher results. 
We have modified the text to make this point clearer (\fpointer{5}{1}{370}).

In addition, we have added a timeline diagram (i.e., 
new Figure~\ref{fig:timeline} in the revised paper) 
to show how each \approach presents \res{s} to the user in the viewport 
in Section~\ref{sec:new_property}. 
We did not use a diagram for different types of consistencies 
because one type of consistency can correspond to different \approaches. 
}

\subsection*{Reviewer \#2}

We have numbered the comments from Reviewer \#2 in sequence.

\Rev{R2.D1}{Before I forget, please change all green colored items in your figures with blue. There are people who cannot discriminate between green and red, and, in such a case, the paper is very hard to follow.
I read on b/w printouts (I suppose revealing the age of the reviewer does not break the secrecy on the reviewer's identity) and, of course, I had to open the pdf in parallel.
But at least, please replace green with blue (equiv: keeping green and changing red would also work)}

\Ans{We have changed the red and green colors to 
gold and blue, respectively.}

\Rev{R2.D2}{One issue I have with the paper is that I am not clear on what the end-user can do. If I get it right, the end user is practically passive: there is a set of charts displayed and the user alternates the viewport of which charts she observes. In case the user performs filters (importantly: removal of filters), pan \& shift, zooms in and out --e.g., over an aggregate chart over a graph, how does this impact the panorama? In extremes, what if the charts are aggregate queries and the user performs drill-down, drill across, etc. There are parts, concerning the different versions of the graph that would have to be computed very quickly, and, also it is unclear how the scheduler would work. Some discussion on this would be appropriate}

\Ans{The focus of this paper is on the 
``passive'' use case where the user can consume and 
move the viewport but not do much more. 
This is the common case of the user continuously consuming 
dashboards, especially in the monitoring and observability setting. 
For the ``active'' case, we show that it is possible 
to extend the \tdb model to support actions beyond 
modifying the viewport and also discuss additional concerns 
that stem from the intended user semantics. This discussion 
is now added in Section~\ref{sec:extension}. 
We discuss extending \tdb 
to support reading and modifying the definition of a \viewG 
(e.g., modifying a filter on a base table via a filter box of a dashboard), 
supporting the aforementioned actions in the extended model, 
and practical concerns regarding the user interface. 

In terms of semantics, the user can read the \vdef if it is rendered 
alongside the corresponding visualization in the viewport, 
so a \readTxn is extended to read \qres{s} and/or \vdef{s} 
in the viewport, depending on which of them 
are rendered in the visualizations. 
To support modifying a \vdef, 
a \viewG's edges and \vdef{s} are multi-versioned; 
that is, a \version of \viewG is defined to be 
$G^{t_i}= (E^{t_i}, \Vt^{t_i}, \Vs^{t_i})$. 
A modification to a \vdef is modeled as a \writeTxn 
that modifies the \vdef and refreshes the visualizations 
that depend on it (e.g., modifying a filter on a base table will 
refresh the visualizations derived from this base table). 
The system and scheduler processes the \writeTxn 
in the same way as processing the \writeTxn that is created by 
modifying the source data. 

To support the new user actions in the extended \tdb model, 
we break them into two broad categories. 
If the user action needs to be processed at the back-end 
(e.g., a web server), where \tdb operates, 
then this user action is interpreted as a \writeTxn that involves 
modifying the \vdef (e.g., modifying a filter). 
Otherwise, if the user action is performed at the front-end 
(e.g., shifting a visualization), 
\tdb does not need to intervene. 

All that said, while supporting the aforementioned actions, 
the visual interface may present the old \vdef 
for some \approach{es} even after  
the user modifies the \vdef  
(e.g., presenting the old value of a filter after 
it is modified for \pGCNB to preserve \con), 
which introduces additional complications 
regarding the desired user experience. 
If, for example, the dashboard designer determines that 
it should not show an old filter value to the user 
after they have updated it --- since that might be confusing to the user, 
then the selected \approach can be overridden to 
be either \pGCPB or \pICNB to process 
the case for modifying and reading a filter. 
For all other cases, the selected \approach will be used. 
%To resolve this issue, we may need additional dashboard 
%designs to notify the user that the related visualizations 
%with respect to the \vdef modification are under computation. 
This discussion is added in Section~\ref{sec:extension}.
}

\Rev{R2.D3}{Section 2.3 and 2.4 -- as well as later in the paper. There are some terms that need to be clarified better. 
"results": IMHO you refer to "view state", or "node state", rather than results per se. If I get it right, this concerns the state of the view, not the contents of the results.
"committed": please be precise with what you mean by the term "committed". As this is not the typical ACID xact manager inside the DBMS, the term commit needs precise definition.}

\Ans{To address the confusion around the term ``results'', 
we have now changed ``query result'' to a new name, ``\qres'', 
which is defined as the output of a given view 
given a version of the source data and \viewG definition 
(\fpointer{3}{2}{230}). 
For what the user sees on reading a view, 
we now call it ``\vstate'', which is 
either a \qres or an under-computation state (\fpointer{3}{2}{243}). 
The detailed text can be found in Section~\ref{sec:bg}. 

In addition, we have now added the definition for 
what it means when we say that a \writeTxn is committed 
at the end of the first paragraph of Section~\ref{sec:formalize} 
(\fpointer{4}{2}{321}).
Specifically, a \writeTxn is defined to be committed 
if the system has computed all of the \qres{s} for 
the version of \viewG created by this \writeTxn, 
and finally updates a global variable that records 
the version of the recently \oldG. 
Section~\ref{sec:cc} discusses the procedure 
for processing a \writeTxn and the management of this global variable.
}

\Rev{R2.D4}{Section 2.6. Lenses. The LCNB is weakly defined. IMHO all definitions should explicitly refer to just ``committed'' or ``latest'' graph version, without any other term used. Or, if need, introduce the terms needed.}

\Ans{In Section~\ref{sec:new_property}, 
we have now refactored the definition of \pLCNB to be the following: 
between the \oldAndNew \viewG{s}, \pLCNB 
reads the most recent \version that 
does not return \ua{s} for any \readTxn, 
thereby ensuring that each viewport does not have \unavailable views 
and that the \res{s} within the viewport are consistent (\fpointer{6}{1}{511}).}

\Rev{R2.D5}{Architecture and Write Transactions. I am not sure whether section 2.2. and Sections 3 \& 4 are in-sync.
If I understand well, the main idea of "write transactions" in Section 2.2 is that the contents of the underlying db are updated.
It is not at all clear (and in fact, it has been a tremendously hard part for data warehouses) how the panorama learns that the contents have changed.
There are 3 fundamental models: on demand (i.e., you change the viewport and you go and issue all the queries for its contents?), on-update (i.e., there is a channel from the db to the panorama informing there is a change), and, the easiest, periodically.
It is not clear to me, in Sections 3 and 4, how the write manager is triggered. I do understand that the scheduler takes care for the internal order, once the write action has been triggered, but how do you decide it is time to trigger the write manager and create a new version of the graph.
IMHO this needs to be crystal clear, as it impacts severely the validity of the experimental section.
}

\Ans{The specific strategy for triggering \writeTxn{s}  
is independent of the \tdb model. 
The \tdb model supports all three models described 
by the reviewer: on-demand (pull), on-update (push), and periodic 
refreshes. Each of the three types of refreshes 
are modeled as a \writeTxn. 
The \tdb model also supports multiple \writeTxn{s} that are created 
by different types of refreshes, possibly interleaved. 
Each of them will be scheduled and executed as usual. 
However, in today's BI tools, such as Superset, 
Tableau, and Power BI, the dashboard is either refreshed manually 
(i.e., on-demand) or configured to refresh periodically (e.g., every 1 min). 
Therefore, in our prototype, we support both manual 
and periodic refresh. 
For the new experiments that test multiple refreshes, 
we use periodic refresh. 
In the revised paper, we have now added a discussion 
for the strategy for triggering \writeTxn{s} 
in Section~\ref{sec:prototype}, 
the prototype implementation, 
added a forward pointer in the first paragraph of Section~\ref{sec:system} 
to note that Section~\ref{sec:prototype} will discuss the strategy 
for triggering \writeTxn{s}, 
and mentioned that we adopt periodic refreshes to test multiple refreshes 
in the new experiment (\fpointer{11}{2}{952}). 
}

\Rev{R2.D6}{Section 6 experiments: right at the start of the section you mention you test one refresh of the data, as it does not impact the relative performance of the different lenses.
I am not sure that this holds. In case you have data too frequently updated, the system needs to create too many versions fast. Whereas the latches that use the committed versions are not stalled, everyone else (esp., intolerant to invisibility) have to wait. 
Maybe I get this wrong, but in my opinion, the rate of updates to the data and the way you handle them play 
a role to the behavior of the system. 
This is why, traditionally, view update algorithms have always had a read/write frequency ratio as an experimental parameter, which, of course, is missing here.
Btw., I don't think that the case of a user that 
moves around a lot in the dashboard is covered by the experiments.}

\Ans{We agree that if there are multiple concurrent \writeTxn{s}, 
the relative performance across different \approach{es} will be different. 
We have added a new experiment to show how the frequency of triggering 
refreshes impacts the relative performance for different \approach{es} 
at the end of Section~\ref{sec:exp_discrete} (\fpointer{11}{2}{952}).
We test three refreshes, where the interval 
between two succeeding refreshes (i.e., \prefreshinterval) 
is varied from 10s to 60s. 
Same as the test for one refresh, before starting each refresh, 
we insert 0.1\% new data to the database. 
We report the \snMetric and \uaMetric 
for different \approach{es}. 
Figure~\ref{fig:exp_refresh_interval} shows 
that a smaller \prefreshinterval introduces 
higher \snMetric and \uaMetric 
when the \prefreshinterval is less than the 
execution time for processing a refresh (i.e., 37s in our test) 
for all \approach{es} except \pGCNB. 
This is because while a \version of the \viewG is being computed, 
a smaller \prefreshinterval creates a new \version of the \viewG earlier. 
This leads the \qres{s} of the under-computation 
\version of the \viewG becoming stale earlier, 
and, in turn the \snMetric and \uaMetric are increased. 
The \snMetric of \pGCNB is not impacted by the varied \prefreshinterval 
because \pGCNB presents the up-to-date \qres{s} 
to the user when it finishes all of the refreshes in the system 
and its \snMetric is determined by the 
execution time for finishing multiple refreshes, 
which is independent of the \prefreshinterval.

We test one refresh for most of the experiments 
since the main focus of this paper 
is on the scenario where there is 
only one \writeTxn in the system at a time. 
This case happens when the period for triggering 
a refresh is longer than the time for executing the refresh 
or the system only processes one refresh at a time (e.g., Tableau). 
For the test of one refresh, 
we insert 0.1\% new data to the tables Lineitem, 
Orders, and PartSupp and then refresh  
all of the 22 visualizations. 
We have now refactored the text to clarify 
the above point in the second paragraph of 
Section~\ref{sec:experiment} (\fpointer{9}{2}{818}). 
Thoroughly studying the performance of concurrent \writeTxn{s}, 
which may stem from multiple users, is left to future work. 

For the case that a user moves around a lot in the dashboard, 
we use the \ranMove behavior 
to simulate it. In our test, we modify the viewport every 1s. 
We have now refactored the text 
in the third paragraph of Section~\ref{sec:experiment} 
to highlight this point (\fpointer{9}{2}{841}).}

\subsection*{Reviewer \#3}

\Rev{R3.W1}{The proposed MVC combinations only have significant difference on invisibility and staleness in such situations: (1) the view port (the region viewed by the user) has many charts (say, >10 as depicted in Fig 14b) shown at the same time (2) the view port is small but the user quickly moves around on the large visualization dashboard. In other words, it is when the screen needs to show many charts at the same time.}

\Ans{When the user explores more visualizations, 
the difference on \uaMetric and \snMetric will become more 
significant across different \approach{es}. 
We have now clarified this point in 
Section~\ref{sec:exp_discrete} (\fpointer{11}{1}{949}).}

\Rev{R3.\{W2, D1\}}{It is unclear that how the invisibility and staleness are measured in the experiments. 
Although Section 2.7 gives the definitions of invisibility and staleness used in this paper, I am still not sure how the invisibility and staleness are measured. Suppose we have a viewport that has many charts, is the invisibility the time between the read transaction starting timestamp (at least a chart becomes invisible) and the read transaction ending timestamp (all charts become visible again)? The same question also applies to the staleness.}

\Ans{We have now clarified how we measure 
\uaMetric and \snMetric in our experiments 
right before Section~\ref{sec:exp_discrete}(\fpointer{10}{1}{866}).
To measure \uaMetric and \snMetric, the test 
client tracks the timestamp when each \readTxn returns the \res{s} 
and the content of the returned \res{s}, 
which include the information regarding whether each returned \res 
is a \ua or a stale \qres. 
Using this information and the definitions in Section~\ref{sec:metrics}, 
we can compute \uaMetric and \snMetric. 
For example, the \uaMetric for one test is initialized to 0. 
During the test, if a \readTxn has returned a \ua for a view, 
then the time difference between when this and 
the next \readTxn return will be added to the \uaMetric. 
Intuitively, this is the duration when this view is \unavailable between 
two consecutive \readTxn{s}.}

\Rev{R3.\{W3, D2\}}{Some writing can be improved. 
The paper uses lots of notations and abbreviations. It should use a table to summarize all of them. I have a hard time tracking all these notations throughout the paper.}

\Ans{We have now added Table~\ref{tbl:notation} 
to summarize the frequently used notation in this paper 
and added the text in the first 
paragraph of Section~\ref{sec:formalize} to refer to this table.}
